Provable Robustness of Adversarial Training for Learning Halfspaces with Noise

We analyze the properties of adversarial training for learning adversarially robust halfspaces in the presence of agnostic label noise. Denoting $\mathsf{OPT}_{p,r}$ as the best robust classification error achieved by a halfspace that is robust to perturbations of $\ell_{p}$ balls of radius $r$, we show that adversarial training on the standard binary cross-entropy loss yields adversarially robust halfspaces up to (robust) classification error $\tilde O(\sqrt{\mathsf{OPT}_{2,r}})$ for $p=2$, and $\tilde O(d^{1/4} \sqrt{\mathsf{OPT}_{\infty, r}} + d^{1/2} \mathsf{OPT}_{\infty,r})$ when $p=\infty$. Our results hold for distributions satisfying anti-concentration properties enjoyed by log-concave isotropic distributions among others. We additionally show that if one instead uses a nonconvex sigmoidal loss, adversarial training yields halfspaces with an improved robust classification error of $O(\mathsf{OPT}_{2,r})$ for $p=2$, and $O(d^{1/4}\mathsf{OPT}_{\infty, r})$ when $p=\infty$. To the best of our knowledge, this is the first work to show that adversarial training provably yields robust classifiers in the presence of noise.

==> l2_normalized.tex <==
\begin{lemma}\label{lemma:upperbound_opt_grad_product}
Let $\wb^*=\arg\min_{\|\wb\|_2=1}L_\cD^{2,r}(\wb)$ be the optimal model parameter that achieves minimum $\ell_2$ robust error and $\err_\cD(\wb^*)$ be the clean error achieved by $\wb^*$. Then for any $\wb$ of $\ell_2$ norm $1$, define by $\theta$ the angle between $\wb^*$ and $\wb$ and $\theta^* = \min\{\arcsin(4r/R), \arcsin(4\sigma/R)\}$, then if $\err_\cD(\wb^*)\le (2^{14}U^2R^4)^{-1}\sigma$ and $\theta\in(\theta^*,\pi-\theta^*)$, it holds that 
\begin{align*}
\wb^{*\top}\nabla L_\cD^{p,r}(\wb)\le -\frac{R^2\sin\theta}{4\pi U}.
\end{align*}
\end{lemma}
\begin{proof}
% \CC{For any constant $z$, $\nabla_{\wb}h(\wb,z) = \bigg(\Ib - \frac{\bar \wb \wb^\top}{\|\wb\|_q^{q}}\bigg)\frac{z}{\|\wb\|_q}$ holds.  Since $\bar \wb^\top w = \|\wb\|_q^q$, for $x^* = x - ry\bar \wb/\|\wb\|_q^{q-1}$, this implies}
% \[ \CC{\frac{\wb^\top\xb^*}{\|\wb\|_q} = \frac{\wb^\top\xb}{\|\wb\|_q} - \frac{r y \bar \wb^\top w}{\|\wb\|_q^q} = \frac{\wb^\top\xb}{\|\wb\|_q} - ry.}\]
% \CC{In particular,}
% \[ \CC{\nabla_{\wb} h(\wb,x^*) = \nabla_{\wb}(h, x - ry \bar \wb/\|\wb\|_q^{-1}) = \nabla \frac{\wb^\top\xb}{\|\wb\|_q} = \frac{\xb}{\|\wb\|_q} - \frac{(\wb^\top\xb) \bar \wb}{\|\wb\|_q^{1+q}}},\]
% \CC{and thus \eqref{eq:strongest.attacker} holds.} 
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figure/diagram_l2.jpg}
\caption{Illustration of the set $G$ and $G^c$. \label{fig:diagram_l2}}
\end{figure}

% leading to an ``effective'' term, corresponding to the data that can be correctly classified by $\wb^*$, and an ``error'' term, which is misclassified by $\wb^*$. Then the inner product $\wb^{*\top}\nabla L_\cD^{p,r}(\wb)$ can be bounded using only the information of $\wb$, $\wb^*$, and the distribution of $\xb$. Since the distribution of $\xb$ is isotropic and satisfies certain nice anti-concentration and anti-anti-concentration properties, defined in Definition \ref{def:anticoncentration}. We can show that as long as $\wb$ is not approaching $\wb^*$ and the clean error achieved by $\wb^*$ is small, the ``effective'' term dominates the ``error'' term and consequently leads to an upper bound on $\wb^{*\top}\nabla L_\cD^{p,r}(\wb)$.

In the $\ell_2$ case, we have $\bar \wb = \wb$. Besides, note that $\|\wb\|_2=1$, we have $\tilde \wb = \wb^* - ( \wb^\top \wb^*)\wb$. Then it is easy to verify that $\tilde \wb^\top \wb = 0$ and $\tilde \wb^\top \wb^*\ge 0$. Then we will focus on the $2$-dimensional space spanned by the vectors $\wb$ and $\wb^*$ (or $\tilde \wb$ since these three vectors lie in the same $2$-dimensional space). Without loss of generality, we assume $\wb$ follows the $Y$-axis and define by $\theta$ 
the angle between $\wb$ and $\wb^*$. We further define the set $G:=\{\xb:\text{sgn}(\wb^{*\top}\xb) = \text{sgn}(\tilde \wb^\top\xb)\}$, which is marked as the shaded region in Figure \ref{fig:diagram_l2},
and $I_1$ can be rewritten as
\begin{align}\label{eq:formula_I1_1}
I_1 &= \EE_{(\xb,y)\sim \cD}\big[g_{S}(\wb^*,\wb;\xb)\cdot \text{sgn}(\wb^{*\top}\xb)\cdot \tilde \wb^\top\xb \cdot (I_G(\xb)+I_{G^c}(\xb))\big]\notag\\
& = \EE_{(\xb,y)\sim \cD}\big[g_{S}(\wb^*,\wb;\xb)\cdot | \tilde \wb^\top\xb |\cdot I_{G}(\xb))\big]-\EE_{(\xb,y)\sim \cD}\big[g_{S}(\wb^*,\wb;\xb)\cdot | \tilde \wb^\top\xb |\cdot I_{G^c}(\xb))\big].
\end{align}
Without loss of generality, we assume $\wb$ lies along the y-axis and $\theta\le \pi/2$. Note that the following proof also holds for the case of $\theta\ge \pi/2$ due the fact that the distribution of $\xb$ is isotropic. Let $p(\xb)$ be the probability density function of the feature $\xb$ and decompose the set $G$ by $G = G_1\cup G_2$, where $G_2 = \{\xb:\angle (\xb, \eb_1)\in[-\theta, \theta]\}$ and $G_1 = G-G_2$. Note that the regions $G^c$ and $G_1$ are symmetric with respect to the vector $\wb$ and $\tilde \wb$ is orthogonal to $\wb$, then we have for any point $\xb$ in $G^c$, there must have an unique point $\xb'$ in $G_1$ such that $\wb^\top\xb'=\wb^\top\xb$, $\text{sgn}(\wb^{*\top}\xb)=\text{sgn}(\wb^{*\top}\xb')$ and $p(\xb) = p(\xb')$ due to the fact that the $p(\xb)$ is isotropic. Combining this further yields that
\begin{align*}
g_{S}(\wb^*,\wb;\xb)\cdot | \tilde \wb^\top\xb | = g_{S}(\wb^*,\wb;\xb')\cdot | \tilde \wb^\top\xb' |.
\end{align*}
Plugging the above equation into \eqref{eq:formula_I1_1} gives
\begin{align*}
I_1 = \EE_{(\xb,y)\sim \cD}\big[g_{S^c}(\wb^*,\wb;\xb)\cdot | \tilde \wb^\top\xb |\cdot I_{G_2}(\xb))\big].
\end{align*}
Let $\bar \xb$ be the projection of $\xb$ onto the space spanned by $\wb$ and $\wb^*$, we can express it in polar coordinates as $\bar \xb = (l\cos\phi, l\sin\phi)$ \todoq{I don't like $l$, any better choice of symbol?}.
Note that the distribution of $\xb$ is isotropic and 
\begin{align}\label{eq:formula_g_sc}
g_{S}(\wb^*,\wb;\xb) &= \ell'(\text{sgn}(\wb^{*\top}\xb)\cdot \wb^\top\xb-r)\notag\\
& = -\frac{e^{-|\text{sgn}(\wb^{*\top}\xb)\cdot \wb^\top\xb-r|/\sigma}}{\sigma}\notag\\
& = -\frac{e^{-|\text{sgn}(\wb^{*\top}\xb)\cdot l\sin\phi-r|/\sigma}}{\sigma},
\end{align}
where the second last inequality is due to the fact that $\wb=\eb_2$. 
Since the distribution of $\xb$ is isotropic, the probability density function of $\bar \xb$ can be formulated as $p(\bar \xb) = \frac{p(l)}{2\pi}$, where $p(l)$ denotes the distribution of the length of $\bar \xb$. Then we have the following regarding $I_1$,
\begin{align}\label{eq:formula_I1_2}
I_1 &= -\frac{1}{\sigma}\int_{0}^\infty \bigg(\int_{-\theta}^{\theta} p(\bar \xb) l^2\|\tilde \wb\|_2|\cos \phi| e^{-|l\sin\phi-r|/\sigma}\dd l\dd \phi + \int_{\pi-\theta}^{\pi+\theta} p(\bar \xb) l^2\|\tilde \wb\|_2|\cos \phi| e^{-|l\sin\phi+r|/\sigma}\dd l\dd \phi\bigg)\notag\\
& = -\frac{\|\tilde \wb\|_2}{\pi\sigma}\int_{0}^\infty p(l)l^2 \dd l \underbrace{\int_{-\theta}^{\theta} |\cos \phi| e^{-|l\sin\phi-r|/\sigma}\dd \phi}_{I_3},
\end{align}
where the second equality holds since $\sin (\pi+\phi) = -\sin\phi$ and $|\cos\phi| = |\cos(\phi+\pi)|$. Further note that $|\cos \phi|=\cos\phi$ when $\phi\in[-\theta,\theta]$, we have
\begin{align*}
I_3& = \int_{-\theta}^{\theta}  \cos \phi e^{-|l\sin\phi-r|/\sigma}\dd \phi \notag\\
& = \int_{-\sin\theta}^{\sin\theta}  e^{-|lz - r|/\sigma}\dd z.
\end{align*}
Then we will need to consider two cases: (1) $l\sin\theta\le r$ and (2) $l\sin\theta\ge r$. In the first case we have 
\begin{align*}
I_3 = \int_{-\sin\theta}^{\sin\theta}  e^{(lz - r)/\sigma}\dd z = \frac{\sigma}{l}\Big(e^{-(r-l\sin\theta)/\sigma}-e^{-(r+l\sin\theta)/\sigma}\Big).
\end{align*}
In the second case we have
\begin{align*}
I_3 &= \int_{-\sin\theta}^{r/l}  e^{(lz - r)/\sigma}\dd z + \int_{r/l}^{\sin\theta}  e^{(r - lz )/\sigma}\dd z \notag\\
&= \frac{\sigma}{l}\Big(2-e^{-(l\sin\theta+r)/\sigma}-e^{-(l\sin\theta-r)/\sigma}\Big).
\end{align*}
Plugging the above calculations for $I_3$ into \eqref{eq:formula_I1_2}, we have
\begin{align*}
I_1 &= -\frac{\|\tilde \wb\|_2}{\pi}\bigg(\int_{0}^{r/\sin\theta} p(l) l\Big(e^{-(r-l\sin\theta)/\sigma}-e^{-(r+l\sin\theta)/\sigma}\Big)\dd l \notag\\
&\qquad + \int_{r/\sin\theta}^{\infty}p(l)l \Big(2-e^{-(l\sin\theta+r)/\sigma}-e^{-(l\sin\theta-r)/\sigma}\Big)\dd l \bigg).
\end{align*}
We will further consider two cases: (1) $\sin\theta\le r/R$ and (2) $\sin\theta\ge r/R$, where $R$ is the constant from Assumption \ref{assump:isotropic}. Regarding the first case, we have 
\begin{align}\label{eq:bound_I1_case1}
I_1 &\le -\frac{\|\tilde \wb\|_2}{\pi U}\int_{0}^{R} l\Big(e^{-(r-l\sin\theta)/\sigma}-e^{-(r+l\sin\theta)/\sigma}\Big)\dd l\notag\\
&=-\frac{\|\tilde \wb\|_2 e^{-r/\sigma} }{\pi U}\int_{0}^{R} l\Big(e^{l\sin\theta/\sigma}-e^{-l\sin\theta/\sigma}\Big)\dd l\notag\\
&\le -\frac{2\|\tilde \wb\|_2 e^{-r/\sigma} }{\pi U}\int_{0}^{R} \frac{l^2\sin\theta}{\sigma}\dd l\notag\\
& = -\frac{2R^3\|\tilde \wb\|_2e^{-r/\sigma}\sin\theta}{3\pi U \sigma},
\end{align}
where the first inequality follows from Assumption \eqref{assump:isotropic} that $p(l)\ge 1/U$ for all $l\le R$ and the second inequality holds since $e^{x}-e^{-x}\ge 2x$ for any $x\ge 0$. Regarding the second case, we have
\begin{align*}
I_1 &\le -\frac{\|\tilde \wb\|_2}{\pi U}\bigg(\int_{0}^{r/\sin\theta} l\Big(e^{-(r-l\sin\theta)/\sigma}-e^{-(r+l\sin\theta)/\sigma}\Big)\dd l \notag\\
&\qquad + \int_{r/\sin\theta}^{R}l \Big(2-e^{-(l\sin\theta+r)/\sigma}-e^{-(l\sin\theta-r)/\sigma}\Big)\dd l \bigg)\notag\\
&\le -\frac{2r^3\|\tilde \wb\|_2e^{-r/\sigma}}{3\sin^2\theta\pi U \sigma} - \frac{\|\tilde \wb\|_2}{\pi U}\int_{r/\sin\theta}^{R}l \Big(1- e^{-(r+l\sin\theta)/\sigma}\Big)\dd l\notag\\
&\le -\frac{2r^3\|\tilde \wb\|_2e^{-r/\sigma}}{3\sin^2\theta\pi U \sigma} - \frac{\|\tilde \wb\|_2}{\pi U}\int_{r/\sin\theta}^{R}l \Big(1- e^{-l\sin\theta/\sigma}\Big)\dd l\notag\\
&\le -\frac{2r^3\|\tilde \wb\|_2e^{-r/\sigma}}{3\sin^2\theta\pi U \sigma} - \frac{\|\tilde \wb\|_2}{\pi UR}\int_{r/\sin\theta}^{R}l^2 \Big(1- e^{-R\sin\theta/\sigma}\Big)\dd l\notag\\
&= -\frac{2r^3\|\tilde \wb\|_2e^{-r/\sigma}}{3\sin^2\theta\pi U \sigma} - \frac{(R^3-r^3/\sin^3\theta)\|\tilde \wb\|_2}{3\pi UR} \Big(1-e^{-R\sin\theta/\sigma}\Big),
\end{align*}
where the first inequality is due to the fact that $p(l)\ge 1/U$ for all $l\le R$, for the second inequality we use \eqref{eq:bound_I1_case1} by setting $R = r/\sin\theta$ and the fact that $1-e^{-(l\sin\theta-r)}\ge 0$, and the last inequality follows the fact that the function $f(x)=(1-e^{-ax})/x$ is strictly decreasing with respect to $x$ for any positive constant $a$ so that we have $1- e^{-l\sin\theta/\sigma}\ge l(1- e^{-R\sin\theta/\sigma})/R$. Combining the previous results we can conclude that 
\begin{align*}
I_1\le \left\{
\begin{array}{lc}
  -\frac{2R^3\|\tilde \wb\|_2 e^{-r/\sigma}\sin\theta}{3\pi U\sigma}   &  \sin\theta\le r/R,\\
   -\frac{2r^3\|\tilde \wb\|_2e^{-r/\sigma}}{3\sin^2\theta\pi U \sigma} - \frac{(R^3-r^3/\sin^3\theta)\|\tilde \wb\|_2}{3\pi UR} \Big(1-e^{-R\sin\theta/\sigma}\Big)  & \sin\theta\ge r/R.
\end{array}
\right.
\end{align*}  
Furthermore, if focusing on the case that $\sin\theta\ge 4r/R$, we have
\begin{align}\label{eq:upperbound_II1}
I_1\le-\frac{3R^2\|\tilde \wb\|_2}{10\pi U}\big(1-e^{-R\sin\theta/\sigma}\big).
\end{align}



Then we will focus on deriving an upper bound of $|I_2|$. Based on Cauchy-Schwarz inequality, we have
\begin{align*}
|I_2| \le \sqrt{\underbrace{\EE_{\xb}\big[\big(g_{S}(\wb^*,\wb;\xb)+g_{S^c}(\wb^*,\wb;\xb)\big)^2\cdot \big(\wb^{*\top}\nabla_{\wb}h(\wb,\xb+\deb)\big)^2\big]}_{I_4}}\cdot\sqrt{\EE_{\xb}[\ind_{S^c}(\xb)]}.
\end{align*}
Based on our definition of the set $S^c$, we have $\EE_x[\ind_{S^c}(\xb)] = \text{err}_D(\wb^*)$. Regarding $I_4$, we substitute the definitions of $g_S(\wb^*,\wb;\xb)$ and $g_{S^c}(\wb^*,\wb;\xb)$ and the fact that $\wb^{*\top}\nabla_{\wb}h(\wb,\xb+\deb) = \tilde \wb^\top\xb$ and obtain
\begin{align*}
I_4 = \frac{1}{\sigma^2}\EE_{\xb}\bigg[\Big(e^{-|\text{sgn}(\wb^{*\top}\xb) \wb^\top\xb +r|/\sigma}+e^{-|\text{sgn}(\wb^{*\top}\xb) \wb^\top\xb-r|/\sigma}\Big)^2\cdot (\tilde \wb^\top\xb)^2\bigg].
\end{align*}
Again using polar coordinate $\bar \xb = (l\sin\phi, l\cos\phi)$, we have $\wb^\top\xb = l\sin\phi$ and $\tilde \wb^\top\xb = l\|\tilde \wb\|_2\cos\phi$. Further note that $e^{-|\text{sgn}(\wb^{*\top}\xb) \wb^\top\xb +r|/\sigma}+e^{-|\text{sgn}(\wb^{*\top}\xb) \wb^\top\xb-r|/\sigma} = e^{-| \wb^\top\xb +r|/\sigma}+e^{-|\wb^\top\xb-r|/\sigma}$ due to the symmetry, we have
\begin{align*}
I_4 &= \frac{\|\tilde \wb\|_2^2}{\sigma^2}\int_{0}^\infty \int_{0}^{2\pi} \Big(e^{-|l\sin\phi +r|/\sigma}+e^{-|l\sin\phi -r|/\sigma}\Big)^2\cos^2\phi p(\bar \xb)l^3 \dd l\dd \phi \notag\\
&=\frac{\|\tilde \wb\|_2^2}{\pi\sigma^2}\int_{0}^\infty p(l)l^3 \dd l \int_{-\pi/2}^{\pi/2} \Big(e^{-|l\sin\phi +r|/\sigma}+e^{-|l\sin\phi -r|/\sigma}\Big)^2\cos^2\phi  \dd \phi \notag\\
&\le \frac{\|\tilde \wb\|_2^2}{\pi\sigma^2}\int_{0}^\infty p(l)l^3 \dd l \int_{-\pi/2}^{\pi/2} \Big(e^{-|l\sin\phi +r|/\sigma}+e^{-|l\sin\phi -r|/\sigma}\Big)^2\cos\phi \dd \phi\notag\\
& = \frac{\|\tilde \wb\|_2^2}{\pi\sigma^2}\int_{0}^\infty p(l)l^3 \dd l \int_{-1}^{1} \Big(e^{-|lz +r|/\sigma}+e^{-|lz -r|/\sigma}\Big)^2\dd z\notag\\
&\le \frac{2\|\tilde \wb\|_2^2}{\pi\sigma^2}\int_{0}^\infty p(l)l^3 \dd l \int_{-1}^{1} e^{-2|lz +r|/\sigma}+e^{-2|lz -r|/\sigma}\dd z\notag\\
& = \frac{4\|\tilde \wb\|_2^2}{\pi\sigma^2}\int_{0}^\infty p(l)l^3 \dd l \int_{-1}^{1} e^{-2|lz +r|/\sigma}\dd z,
\end{align*}
where in the second equality we use $p(\bar\xb) = p(l)/(2\pi)$, the first inequality follows from the fact that $\cos^2\phi\le \cos\phi$ for all $\phi\in[-\pi/2, \pi/2]$ and the last inequality is by Young's inequality. 
Similar to previous analysis, we will consider two cases: (1) $l\le r$ and (2) $l\ge r$. In the first case, we have
\begin{align}\label{eq:bound_I4_l2_case1}
\int_{-1}^1 e^{-2|lz+r|/\sigma}\dd z = \int_{-1}^1 e^{-2(lz+r)/\sigma} \dd z = \frac{\sigma}{2l}\Big(e^{-2(r-l)/\sigma} - e^{-2(r+l)/\sigma}\Big)\le \frac{\sigma}{2l}. 
\end{align}
In the second case, we have
\begin{align}\label{eq:bound_I4_l2_case2}
\int_{-1}^1 e^{-2|lz+r|/\sigma}\dd z&=\int_{-1}^{-r/l} e^{2(lz+r)/\sigma}\dd z + \int_{-r/l}^1 e^{-2(lz+r)/\sigma}\dd z \notag\\
& = \frac{\sigma}{2l}\Big(2-e^{-2(l-r)/\sigma}-e^{-2(l+r)/\sigma}\Big)\notag\\
&\le \frac{\sigma}{l}.
\end{align}
Combining the above results, we have
\begin{align*}
I_4&\le \frac{4\|\tilde \wb\|_2^2}{\pi\sigma}\int_{0}^\infty p(l)l^2 dl\le \frac{8\|\tilde \wb\|_2^2}{\pi\sigma}
% \frac{2\|\tilde \wb\|_2^2}{\pi\sigma}\bigg[\int_{0}^r \Big(e^{-2(r-l)/\sigma} - e^{-2(r+l)/\sigma}\Big) p(l)l^2\dd l + \int_{r}^\infty\Big( 2-e^{-2(l-r)/\sigma}-e^{-2(l+r)/\sigma}\Big) p(l)l^2\dd l \bigg]  \notag\\.
\end{align*}
where the inequality is by Assumption \ref{assump:isotropic} that the covariance matrix of $\xb$ is identity so that $\EE_{l\sim p(l)}[l^2] = 2$ ($l$ is the length of the projected vector on a $2$-dimensional space).
This further implies that 
\begin{align*}
|I_2|\le \sqrt{I_4\cdot \err_{\cD}(\wb^*)}\le \frac{2\sqrt{2}\|\tilde \wb\|_2}{\sqrt{\pi}}\cdot\sqrt{\frac{\err_{\cD}(\wb^*)}{\sigma}}.
\end{align*}

Combining the above inequality with $I_1$, we have if $\sin\theta\ge 2r/R$,
\begin{align*}
\wb^{*\top}\nabla L_{\cD}^{\cA}(\wb) \le I_1 + |I_2| \le -\frac{3R^2\|\tilde \wb\|_2}{10\pi U}\big(1-e^{-R\sin\theta/\sigma}\big) + \frac{2\sqrt{2}\|\tilde \wb\|_2}{\sqrt{\pi}}\cdot\sqrt{\frac{\err_{\cD}(\wb^*)}{\sigma}}.
\end{align*}
Then if we also have $\sin\theta\ge 4\sigma/R$ and $\err_{\cD}(\wb^*)\le \sigma/(2^{14}U^2R^4)$, it holds that
\begin{align*}
\wb^{*\top}\nabla L_{\cD}^{2,r}(\wb) \le -\frac{R^2\|\tilde \wb\|_2}{4\pi U},
\end{align*}
which completes the proof.



% Recall $\tilde \wb$ is defined by $\tilde \wb = \wb^*/\|\wb\|_2 - (\bar \wb^\top \wb^*)w/\|\wb\|_2^{3}$, it holds that
% \begin{align*}
% \|\tilde \wb\|_2 = |\wb^{*\top}\tilde \wb| = \frac{\|\wb\|_2^2 - ( \wb^{*\top} w)^2}{\|\wb\|_2^3}
% \end{align*}
\end{proof}

